Transverse Single Spin Asymmetries and Cross-Sections for Forward pi0 and eta Mesons at Large Feynman-x in sqrt(s)=200 GeV polarized p+p Collisions at STAR

The STAR collaboration has previously reported a large transverse single spin asymmetry, A_N, for forward pi0 meson production. The cross-section in this region was measured up to Feynman-x (xF) of 0.55, and found to be consistent with perturbative Quantum Chromo-Dynamics predictions. During RHIC running in the year 2006 (6.8 inverse-pb, 56 % average polarization), an even larger A_N was observed for the eta meson at forward rapidity for xF > 0.5. All data were collected by the STAR Forward Pion Detector during sqrt(s) = 200 GeV polarized p+p collisions at RHIC. Understanding these large spin asymmetries requires information on the production cross-section. In this thesis, we present the results of the cross-section as well as the A_N measurements for both pi0 and eta mesons at average pseudo-rapidity of 3.7, for 0.4 < xF < 0.75. The details of the calibration, and the analysis methods are also discussed. Finally, we present selected aspects of the high voltage system for the STAR Forward Meson Spectrometer inner calorimeter, which was designed primarily by the author and his thesis advisor.

==> SupplementaryMaterial/Dedication.tex <==


To my wife Doeun, for her time independent love and support. \\
To our daughter Serina, for her life and joy.

==> SupplementaryMaterial/ListOfSymbols.tex <==
% Place the list of symbols below.
\begin{eqlist}[\def\makelabel#1{\hfill#1}\labelsep 1em]

\item[$\alpha$]
The first greek letter, p.~\pageref{}

\item[$\alpha$]
The first greek letter, p.~\pageref{}

\item[$\alpha$]
The first greek letter, but we should really add some more text, though we need it to go on two lines, p.~\pageref{}

\item[$\alpha$]
The first greek letter, p.~\pageref{}

\item[$\alpha$]
The first greek letter, p.~\pageref{}

\item[$\alpha$]
The first greek letter, p.~\pageref{}

\item[$\alpha$]
The first greek letter, p.~\pageref{}

\item[$\alpha$]
The first greek letter, p.~\pageref{}

\end{eqlist}
